D3Net: A Unified Speaker-Listener Architecture for 3D Dense Captioning and Visual Grounding

Recent studies on dense captioning and visual grounding in 3D have achieved impressive results. Despite developments in both areas, the limited amount of available 3D vision-language data causes overfitting issues for 3D visual grounding and 3D dense captioning methods. Also, how to discriminatively describe objects in complex 3D environments is not fully studied yet. To address these challenges, we present D3Net, an end-to-end neural speaker-listener architecture that can detect, describe and discriminate. Our D3Net unifies dense captioning and visual grounding in 3D in a self-critical manner. This self-critical property of D3Net also introduces discriminability during object caption generation and enables semi-supervised training on ScanNet data with partially annotated descriptions. Our method outperforms SOTA methods in both tasks on the ScanRefer dataset, surpassing the SOTA 3D dense captioning method by a significant margin.

==> figures/listener.tex <==
\begin{figure}[!h]
    \vspace{-7pt}
    \centering
    \includegraphics[width=0.99\linewidth]{assets/listener.pdf}
    \vspace{-7pt}
    \caption{Listener architecture. We will include it in the paper.}
    \label{fig:listener}
    \vspace{-7pt}
\end{figure}

==> sections/extra.tex <==
\subsection{3D Object Detection}

The field of 3D object detection has attracted research attentions in the past few years~\citep{qi2019deep, hou20193d, hou2020revealnet, chang2017matterport3d, dai2017scannet, hua2016scenenn, song2015sun}. Methods that directly operates on point clouds has achieved great success for their efficiency and effectiveness~\citep{qi2019deep, qi2020imvotenet, cheng2021back, qi2018frustum}. meanwhile, alternative methods that take voxel grids as input achieve impressive performance too~\citep{hou20193d, hou2020revealnet, lahoud20193d, narita2019panopticfusion, engelmann20203d, graham20183d}. Empowered by sparse convolution, voxel-based methods like PointGroup~\citep{jiang2020pointgroup} and 3D-MPA~\citep{engelmann20203d} are enabled to operate on voxel grids with high resolution. This enhances the extracted position-wise features due to enriched visual cues and subsequently improves the quality of detection/segmentation. Our method follows~\citet{jiang2020pointgroup} and use the same spirit to process the voxelized scenes geometry. As color information is critical for describing or localizing objects in the scene, we also utilize the image features encoded via ENet~\citep{paszke2016enet} from the original RGB-D video sequence and back-project them to voxel grids.


